How Did This Get Funded?! Automatically Identifying Quirky Scientific Achievements

Humor is an important social phenomenon, serving complex social and psychological functions. However, despite being studied for millennia humor is computationally not well understood, often considered an AI-complete problem. In this work, we introduce a novel setting in humor mining: automatically detecting funny and unusual scientific papers. We are inspired by the Ig Nobel prize, a satirical prize awarded annually to celebrate funny scientific achievements (example past winner: "Are cows more likely to lie down the longer they stand?"). This challenging task has unique characteristics that make it particularly suitable for automatic learning. We construct a dataset containing thousands of funny papers and use it to learn classifiers, combining findings from psychology and linguistics with recent advances in NLP. We use our models to identify potentially funny papers in a large dataset of over 630,000 articles. The results demonstrate the potential of our methods, and more broadly the utility of integrating state-of-the-art NLP methods with insights from more traditional disciplines.

==> modules/Ensamble.tex <==
% Results suggest the possibility that our estimators have different speciality domains. To utilize models' regions of speciality, we created a stacking ensemble, denoted as ``Iggy''. Its input are the certainty scores of each estimator in the label ``funny'' for a title, along with some intuitive features (e.g., sentence length, polarity, sentiment, AoA). Its output is a single score, indicating the ``Ig-Nobel-worthiness'' of the paper. Our hypothesis was that such an ensemble will increase performance across all fields by accounting for the inconsistency across them of each estimator alone. Iggy is a Multi-layer Perceptron classifier. Training process was as following: we first trained the models on a subset of the data, then, we trained the ensemble on a different subset. Finally, we test it on a new, unseen subset of the data. Pipline of the model is presented in \ref{fig:pipline}. 

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{pipline_iggy.png}
%   \caption{Iggy's pipline}
%   \label{fig:pipline}
%   \Description{Pipline of the ensemble model}
% %   https://www.draw.io/#G1AK78wxX4k4TU3dpr38KnmBmKCdaws9fp
% \end{figure}

% \subsection{Results On The Preliminary Experiments}
% As a first validation of the ensemble, we tested it on the same two initial experiments (our dataset and Ig Nobel retrieval). For this purpose we splitted the dataset to three: train for the models, train for the ensemble and test sets with sizes $70\%, 20\%, 10\%$, respectively. Result can be seen in tables \ref{tab:ensmble_our_dataset} and \ref{}. \cnote{The ensemble isn't much better than sciBERT. Need to explain this.}

\begin{table}[t!]
\caption{Phase one: normalized discounted cumulative gain of the four models for each scientific field on the top 50 rated papers.}
\label{tab:NDCG1}
 \begin{tabular}{l|l|c|c|c|c}
    {} & {} & BERT & SciBERT & Iggy & BERT-Iggy \\
  \bottomrule
  \multirow{5}{*}{Strict} &  &  &  &  &  \\
   {} & Neuroscience     & 0.756 & 0.801 & 0.756 & \textbf{0.852} \\
   {} & Medicine         & 0.675 & \textbf{0.734} & 0.712 & 0.719 \\
   {} & Exact Sciences   & 0.764 & 0.756 & 0.705 & \textbf{0.771} \\
   {} & Biology          & 0.764 & \textbf{0.801} & 0.734 & \textbf{0.801} \\
   {} & All fields       & 0.739 & 0.773 & 0.727 & \textbf{0.786} \\
      \bottomrule

    \multirow{5}{*}{Relaxed} &  &  &  &  &  \\
   {} & Neuroscience     & 0.845 & 0.911 & 0.845 & \textbf{0.963} \\
   {} & Medicine         & 0.749 & 0.852 & 0.83 & \textbf{0.867} \\
   {} & Exact Sciences   & 0.823 & 0.875 & 0.852 & \textbf{0.882} \\
   {} & Biology          & 0.926 & 0.948 & 0.911 & \textbf{0.978} \\
   {} & All fields       & 0.836 & 0.897 & 0.859 & \textbf{0.922} \\
    
\end{tabular}
\end{table}


Our main motivation of this paper is to recommend papers worthy of an Ig Nobel prize. In this section, we test the models that showed promise in Section \ref{sec:pre_exp} towards this goal.

%important experiment we conducted is aimed to measure the performance of the four models described above on a large, more representative, corpus of scientific papers. The importance of this experiment, of course, is to quantify the ability of our models to recommend on good candidates for the longed Ig Nobel award. We will now present the experiment and its results. 

\subsection{Experimental Setup}

We downloaded from Allen Institute's Semantic Scholar\footnote{\url{https://api.semanticscholar.org/corpus}}  $90M$ scientific articles. After some preprocessing and paper-to-field matching (as described in section \ref{sec:dataset}), we were left with $125k-165k$ papers in each field. 
We computed the funniness score using the four best models and used these scores to construct four rankings per title. %We than continue only with the funniest ranked k papers for each field. 
%For each model in , where small Iggy has the same architecture as big Iggy but its input includes only BERT, SCI-BERT, BIO-BERT and the scientific field.

% we sampled from each field in the above mentioned fields. Sample was random according to the minimal between: 50,000 papers or the maximal amount of papers in this field. We used our model to classify all papers in this subset and rank them according to level of certainty in the given label. We than continue only with the highest ranked k papers for each field (only for papers that were classified as funny). We repeated the same procedure for different eight models, were four of them were to use as baselines and the other four can be divided to two models (BERT and sci-BERT based) and their ablation. The four baselines are: dale chall readability, ranking based on the 120,000 words annotation from \cite{gultchin2019humor} (denoted as "Gultchin baseline"), BERT and sci-BERT.

Note that the amount of papers in this experiment is over half a million. Naturally, we did not have labels for them all. Instead,
we used Amazon Mechanical Turk (MTurk) crowdsourcing platform to assess the performance of the models.

\noindent \textbf{Designing the Task.\ }
In an exploratory study we conducted, we asked people to rate the funniness of titles on a Likert scale of 1-5. However, we noted that people tended to confuse funny \emph{research topic} and funny \emph{title}. For example, papers title like ``Are you certain about SIRT?'' or ``NASH may be trash'' received high scores, even though the research topic is not even clear from the title.
%
To mitigate the problem, we designed the experiment to include \emph{two questions}: 1) whether the title is funny, and 2) whether the research topic is funny, both on a 5-point Likert scale. 

For the experiment, conducted through MTurk, we paid workers $\$0.04$ per title. As this is a challenging task, we composed a qualification test with 8 titles (16 questions), allowing for one mistake. The source code for the task and qualification test can be found in the repository\footnote{https://anonymous.4open.science/r/efd424ea-b8fc-43ae-8344-deffc418425a}. We also required workers to have completed at least $1000$ approved HITs with at least $97\%$ success rate. 

The addition of the second question seems to have indeed helped workers understand the problem better. For example, the paper ``Hat-wearing patterns in spectators attending baseball games: a 10-year retrospective comparison'' was marked as serious title, funny topic. The paper ``Slicing the psychoanalytic pie: or, shall we bake a new one? Commentary on Greenberg'' was marked as funny title and serious topic. These examples and others show us that this distinction was understood by the workers.

We also included honeypot questions (labeled examples from our dataset),  further validate that the workers understand the task properly.

Overall, we had $40$ different workers that passed all the qualifications and annotated the data for our experiment. Each worker annotated on average $143.7$ titles, with STD of $244.4$ and median of $24.5$ (the distribution is very far from normal).  We also measured the agreement between workers for the binary humor classification of the title and the research topic (in a binary manner where $1-2 = $ not funny and $3-5 = $ funny). %The binary fleiss kappa sores are: $0.1254$ for title and $0.248$ for topic. \dnote{wait, this is really low. are you sure these are the results?}\nnote{I think that its so low because we have only 3 workers per hit, I think that this kappa isn't very suited for this} This shows us that the humorous level of a title is, in a sense, an easier task than the humorous level of a research topic. 
%\dnote{well, if you don't think it's suited don't report it}



\begin{table}[t!]
\caption{Phase two: normalized discounted cumulative gain of the two best models for each scientific field on the top 200 rated papers.}
\label{tab:NDCG2}
 \begin{tabular}{l|l|c|c}
   \multicolumn{2}{c|}{}&  SciBERT & BERT-Iggy \\
  \bottomrule
    \multirow{5}{*}{Strict} &  &  & \\
   {} & Neuroscience     & \textbf{0.755} & 0.751 \\
   {} & Medicine         & \textbf{0.714} & 0.707 \\
   {} & Exact Sciences   & 0.707 & \textbf{0.731} \\
   {} & Biology          & 0.727 & \textbf{0.740} \\
   {} & All fields       & 0.719 & \textbf{0.731} \\
   \bottomrule
    \multirow{5}{*}{Relaxed} &  &  &  \\
   {} & Neuroscience     & 0.886 & \textbf{0.902} \\
   {} & Medicine         & 0.851 & \textbf{0.858} \\
   {} & Exact Sciences   & 0.869 & \textbf{0.889} \\
   {} & Biology          & 0.910 & \textbf{0.919} \\
   {} & All fields       & 0.874 & \textbf{0.890} \\
\end{tabular}
\end{table}

As a sanity check, we computed Spearman correlation between responses to the first (title) question and the second (topic) question, for each title. We measured this in two manners -- continuous (using the raw, $1-5$ scale annotations) and binary. The Spearman correlation for the continous case is $0.595$ and in the binary case is $0.684$, both with p-values $<10^{-5}$. %\dnote{0? huh?}\nnote{Yes, it was so small that python couldn't handle it and just displayes 0. How should we display this?}



\remove{
\dnote{nevermind, not important enough}
\begin{figure}[h]
  \centering
  \label{fig:MTurk_hist}
  \includegraphics[width=1.05\linewidth]{MTurk_hist.png}
  \caption{Histogram of the number of unique HITs per worker for the MTurk experiment. \cnote{Bigger buckets, more informative x axis and label the axes. }}
\end{figure}
}


\subsection{Results}

We first compared the four best-performing models in the preliminary experiments (BERT, SciBERT, Iggy and BERT-Iggy) by selecting the 50 top-rated papers from each scientific field according to each model. Each title was annotated by three workers.

We measured accuracy using Normalized Discounted Cumulative Gain (NDCG), which is a measure of ranking quality mainly used in information retrieval to quantify the usefulness of an element based on its position in the result list. 
We turned the three rating per title into one binary decision whether the title is humorous or not. We did this in two different scenarios: in the ``strict'' one, a title was classified as funny only if two or more out of the three annotators classified it as `3' or above (on a scale of 1-5 where `1' means `not funny'). In the ``relaxed'' scenario, we relaxed the majority vote decision,   and classified title as `funny' if only one annotator marked it as `3' or above. 

The NDCG of the four models for the top 50 papers for the two scenarios (phase one) is shown in table \ref{tab:NDCG1}. BERT-Iggy is clearly superior, with an average score of $0.786$ and $0.922$, for the strict and relaxed senarious, respectively. A possible explanation for the fact that it outperformed Iggy (which received the same input and more) is that Iggy had more parameters to optimize on a relatively small size of data.   Our second best-performing model is SciBERT, achieving a score of $0.727$ for the strict scenario and $0.897$ for the relaxed one.

\noindent \textbf{Digging Deeper.\ }
In phase two of the experiment we decided to take a closer look at the performance of our top-two models, BERT-Iggy and SciBERT. Therefore, we sent to Mechanical Turk the top 200 and the bottom 50 rated papers for each for each field, for a total of 2000 titles. The bottom 50 papers was used as another sanity check, to ensure that the bottom of the ranking is indeed not funny. Results show that indeed, this is the case -- in the strict settings, 41\% of the top 50 titles were classified as funny, whereas only one of the bottom 50 titles were classified as such. Similarly, in the relaxed case, 76\% of the top 50 papers and 10\% of the bottom 50 papers were considered funny. Results of phase two of the experiment can be seen in table \ref{tab:NDCG2}. 

We have also considered precision@k (see figure \ref{fig:prec@k}). This graph shows the precision of top rated $k$ titles as a function of $1 \leq k \leq 200$ for the best two models (in both the strict and relaxed scenarios). We measured precision as the cumulative mean of the binary version (three-sized vector to a scalar) of the annotations (step size of $10$ for a smooth, more informative, curve). 
As expected, the precision tends to go down as k increases.
%( \dnote{explain what the reader is supposed to get from this. also, NDCG for 200?}  Results show a clear winner -- BERT-Iggy \cnote{Strict: $0.247 - 0.75$ for sciBERT and $0.296 - 1$ for BERT-Iggy without the jumps, $0.248 - 0.45$ for sciBERT and $0.285 - 0.5$ for BERT-Iggy with the jumps. Relaxed: $0.661 - 0.875$ for sciBERT and $0.707 - 1.0$ for BERT-Iggy without the jumps, $0.667 - 0.799 $ for sciBERT and $0.711 - 0.825$ for BERT-Iggy with the jumps. \textbf{How do you want to report this?}}. \dnote{absolute scores!!!}.
Table \ref{tab:sample} shows a sample of top rated papers found by our winning method. The method indeed managed to identify very funny papers. 
% \begin{table*}[t!]
% \caption{Phase one: normalized discounted cumulative gain of the five models for each scientific field on the top 50 rated papers. \cnote{delete the top left line}}
% \label{tab:NDCG1}
%  \begin{tabular}{l|l|c|c|c|c|c}
%     {} & {} & RF & BERT & SCI-BERT & Iggy & small Iggy \\
%   \bottomrule
%     \multirow{5}{*}{Strict} &  &  &  &  &  &  \\
%   {} & Neuroscience     & 0.683 & 0.845 & 0.911 & 0.845 & \textbf{0.963} \\
%   {} & Medicine         & 0.653 & 0.749 & 0.852 & 0.83 & \textbf{0.867} \\
%   {} & Exact Sciences   & 0.683 & 0.823 & 0.875 & 0.852 & \textbf{0.882} \\
%   {} & Biology          & 0.734 & 0.926 & 0.948 & 0.911 & \textbf{0.978} \\
%   {} & All fields       & 0.688 & 0.836 & 0.897 & 0.859 & \textbf{0.922} \\
%   \bottomrule
%     \multirow{5}{*}{Relaxed} &  &  &  &  &  &  \\
%   {} & Neuroscience     & 0.653 & 0.756 & 0.801 & 0.756 & \textbf{0.852} \\
%   {} & Medicine         & 0.638 & 0.675 & 0.734 & 0.712 & \textbf{0.719} \\
%   {} & Exact Sciences   & 0.638 & 0.764 & 0.756 & 0.705 & \textbf{0.771} \\
%   {} & Biology          & 0.653 & 0.764 & \textbf{0.801} & 0.734 & \textbf{0.801} \\
%   {} & All fields       & 0.646 & 0.739 & 0.773 & 0.727 & \textbf{0.786} \\
% \end{tabular}
% \end{table*}
% 


% \begin{table}[t!]
% \caption{Accuracy of the top and bottom rated 50 according to BERT Iggy and sciBERT. This was done as a sanity check. \dnote{no need for a table -- just report in the text, it's 4 numbers}}
% \label{tab:sanity}
%  \begin{tabular}{l|c|c}
%     {} & Top 50 & Bottom 50 \\
%   \bottomrule
%     Strict     & 0.410 & 0.000 \\
%   Relaxed      & 0.763 & 0.100 \\
% \end{tabular}
% \end{table}






% \subsection{A Closer Look at Our Two Top-Performing Models}

% After discovering the top models for our humor classification, we were curious to see how many of the top results were good. Therefore, we plotted precision of the model for the top k ranked titles as a function of k (see figure \ref{fig:prec@k}). \cnote{\textbf{Do we really want to talk about SHAP? since we're looking at the small ensemble it's not really interesting.}}
% % Another investigation

\begin{figure}[h]
  \centering
  \includegraphics[width=1.05\linewidth]{prec@k.png}
  \caption{Precision of the top two models (BERT-Iggy and SciBERT) for the top k ranked titles as a function of k for the strict and relaxed scenarios.}
  \label{fig:prec@k}
\end{figure}

% In order to gain further understanding of our humor classifier, we turned to investigate it. We started by creating a correlation matrix of all the models, including the ensembles \dnote{weird flow. why is this a way to undersand Iggy-BERT?}. The next step was to use SHAP, a cooperative game theory based analysis created to unravel the average contribution of each feature to the final prediction of small Iggy \cite{lundberg2017unified}.


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=1.05\linewidth]{decision_plot_head_40.png}
%   \caption{Visualization on Iggy's decisions using cumulative SHAP values. Each colored line in the plot represents the model prediction for a single title. \dnote{none of your figures have readable text in them. text shouldn't be smaller than caption size}}
% \end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=1.05\linewidth]{summary_plot_head_4000.png}
%   \caption{SHAP visualization performed on the Iggy. This analysis indicates the average affect of every feature in the Iggy's final prediction.}
% \end{figure}


% ``Epidemiology of Injuries in High School Football: Does School Size Matter?'', ``The deathly hallows: Harry Potter and adolescent development'', ``Baboons, like humans, solve analogy by categorical abstraction of relations'', ``Enjoying vs. smiling: Facial muscular activation in response to emotional language'', ``A freezing-like posture to pictures of mutilation'', ``Smiles make it easier and so do frowns: masked affective stimuli influence mental effort'', ``Physically violent husbands of the 1890s and their resources'', ``Diversion of medical marijuana: when sharing is not a virtue'', ``The ability to self-tickle following Rapid Eye Movement sleep dreaming'', ``Friends don't let friends eat cookies: Effects of restrictive eating norms on consumption among friends'', ``Why stereotypes don’t even make good defaults'', ``Sex and shame: the inhibition of female desire'', ``Hands-on Killing of Intimate Partners as a Function of Sex and Relationship Status/State'', ``Sex, beauty, and the relative luminance of facial features'', ``Emotional and uncontrolled eating styles and chocolate chip cookie consumption. A controlled trial of the effects of positive mood enhancement'', ``Oddity learning by African dwarf goats (Capra hircus)'', ``Moderating effect of ear preference on personality in the prediction of sales performance'', ``Science fiction reduces the eeriness of android robots: A field experime'',  ``What if they knocked down the library and nobody noticed? The failure to detect large changes to familiar scenes'', ``Relative quantity judgment by Asian elephants (Elephas maximus)'', ``Effect of obstacle position in the flow of sheep through a narrow door'', ``Young unmarried men's understanding of female hormonal contraception'', ``Whether to attack a terrorist's resource stock today or tomorrow'', `Nasty online comments anger you more than me, but nice ones make me as happy as you'', ``Time to turn the other cheek? The influence of left and right poses on perceptions of academic specialisation'', ``Feel your food. The influence of tactile sensitivity on picky eating in children'', ``Can seeking happiness make people unhappy? Paradoxical effects of valuing happiness'', ``Uncorking the muse: Alcohol intoxication facilitates creative problem solving'', `Infant cry reliability: Acoustic homogeneity of spontaneous cries and pain-induced cries'', ``Sweetness but not sourness enhancement increases acceptance of cucumber and green capsicum purees in child'', `Odor attributes change in relation to the time of the year. Cinnamon odor is more familiar and pleasant during Christmas season than summertime'', ```Should children drink more water?: The effects of drinking water on cognition in children'', ``Sport is not always healthy: Executive brain dysfunction in professional boxers"" , ``Disgusting smells cause decreased liking of gay men'',

% \begin{enumerate}
%     \item ``On the Separation of Coconuts: A Modeling Week Study''
%     \item ``Women's working wardrobes: a study using card sorts''
%     \item ``Cut of Clothes Maximizes the Effect of Amodal Completion to Make You Look Thinner''
%     \item ``Twisted Lines : Artificial muscle and advanced instruments can be formed from nylon threads and fabric''
%     \item ``Do Androids dream of electric steeds?: the allure of horse-computer interaction''
%     \item ``Looking like mother makes mallard ducklings dominant over their siblings''
%     \item ``A lover, not a fighter: mating causes male crickets to lose fights''
%     \item ``Do bonobos say NO by shaking their head?''
%     \item ``A note on the activities of a solitary male baboon''
%     \item ``Why Don't Chimpanzees in Gabon Crack Nuts?''
%     \item ``Popcorn worker's lung in Britain in a man making potato crisp flavouring''
%     \item ``Metaphoric Car Drawings By a 12-Year-Old Congenitally Blind Girl''
%     \item ``The cheek of a cheater: Effects of posing the left and right hemiface on the perception of trustworthiness''
%     \item ``Singing proficiency in the majority: normality and "phenotypes" of poor singing''
%     \item ``The kinematics of eating with a spoon: bringing the food to the mouth, or the mouth to the food?''
%     \item ``Baby cries and nurturance affect testosterone in men''
%     \item ``EEG activity in Carmelite nuns during a mystical experience''
%     \item ``An Unusual Case of Self-Injected Bovine Fat in Liquid Form to the Face for Cosmetic Reasons''
% \end{enumerate}{}


% \begin{itemize}
%     \item ``Understanding the concept of a reflective surface: Can sheep improve navigational ability through the use of a mirror?''
%     \item ``I Can Use a Condom, I Just Don't: The Importance of Motivation to Prevent HIV in Adolescent Seeking Psychiatric Care''
%     \item ``The effect of pistachio shells as a visual cue in reducing caloric consumption''
%     \item ```Goats that stare at men' – revisited: Do dwarf goats alter their behaviour in response to eye visibility and head direction of a human?''
%     \item ``X-ray scan shows oldest known bird had a bird brain''
%     \item ``Influence of luminance distribution on the appetizingly fresh appearance of cabbage''
%     \item ``More about brows: how poses that change brow position affect perceptions of gender''
%     \item ``Lexicon size and its relation to foot preference in the African Grey parrot''
%     \item ``The influence of hunger on perception of the smell of petrol''
%     \item ``Gorillas in our midst: sustained inattentional blindness for dynamic events'' \cnote{That's the paper with the video of basketball players playing with the Gorilla that most people missed, maybe should mention it because no one will notice...}
%     \item ``The Visual Aesthetics of Snowflakes'' \cnote{First row of the abstract: "In two experiments, participants evaluated the perceived beauty of snowflakes and solid objects."}
%     \item ``Domestic horses send signals to humans when they face with an unsolvable task''
%     \item ``Being Hungry Affects Oral Size Perception''
%     \item ``Cognitive advantages of chewing gum. Now you see them, now you don't''
%     \item ``Do weather, day of the week, and address affect the rate of attempted suicide in Hong Kong?''
%     \item``Humans attribute emotions to a robot that shows simple behavioural patterns borrowed from dog behaviour''
%     \item ``Baboons, like humans, solve analogy by categorical abstraction of relations''
% \end{itemize}{}
% \cnote{keep 5}



\begin{table}[t!]
\caption{ A sample of top rated papers found by our winning model}
\small 
\begin{tabular}{p{\linewidth}}
  \toprule
   ``On the Separation of Coconuts: A Modeling Week Study''\\
    %  ``Women's working wardrobes: a study using card sorts''\\
    %  ``Cut of Clothes Maximizes the Effect of Amodal Completion to Make You Look Thinner''\\
     ``Twisted Lines : Artificial muscle and advanced instruments can be formed from nylon threads and fabric''\\
     ``Do Androids dream of electric steeds?: the allure of horse-computer interaction''\\
    %  ``Looking like mother makes mallard ducklings dominant over their siblings''\\
     ``A lover, not a fighter: mating causes male crickets to lose fights''\\
     ``Do bonobos say NO by shaking their head?''\\
     ``A note on the activities of a solitary male baboon''\\
     ``Why Don't Chimpanzees in Gabon Crack Nuts?''\\
    %  ``Metaphoric Car Drawings By a 12-Year-Old Congenitally Blind Girl''\\
     ``The cheek of a cheater: Effects of posing the left and right hemiface on the perception of trustworthiness''\\
     ``Singing proficiency in the majority: normality and "phenotypes" of poor singing''\\
     ``The kinematics of eating with a spoon: bringing the food to the mouth, or the mouth to the food?''\\
    %  ``Baby cries and nurturance affect testosterone in men''\\
     ``EEG activity in Carmelite nuns during a mystical experience''\\
    %  ``An Unusual Case of Self-Injected Bovine Fat in Liquid Form to the Face for Cosmetic Reasons''\\
   \bottomrule
\end{tabular}
 \label{tab:sample}
\end{table}




==> modules/Methodology.tex <==
Based on the insight that titles are sufficient for our scientific humor detection task, our aim is to create a classifier to distinguish between funny and unfunny papers, based solely on their \emph{titles}. We explored multiple approaches towards creating such a model. 

% After investigating preliminary results of this classifier and baselines we realized an ensemble is needed in order to account for the different regions of specializations of the models. 


% The input to the classifier is a list of $N$ titles along with their scientific field, and its output is a ranked list of size $\leq N$, sorted according to the level of certainty in the label "funny". Our classifier harnesses both past results from the literature and also state-of-the-art techniques in NLP; From each title, we extract local features that are based on well established theoretical and empirical results in humor study. Then, we feed those features, among with the original title, to a Neural Network (NN) that is based on the state-of-the-art BERT architecture \cite{devlin2018bert} to classify each title. \cnote{bert is the pre-trained model, Tranformer is the architecture}

% Our features, since based on soil ground, contribute much for the classification task. Having that said, they are limited in the sense that they represent \emph{local} features of the title, whereas BERT represent it's \emph{holistic} features. Therefore, combining the two led to better results that also mimics human thinking better. Our full model will be described in details shortly, but before we'd like to introduce our dataset.

% The continuation of this section is constructed as follows. First, we introduce the first-of-its-kind dataset which we created specifically for this task. Then, we detail the features that we extract from each title. Finally, we describe the classifier and the NN architecture that it is based on.  


\subsection{Data-Driven Approaches}

%As promising as this retro use of logical rules might be, this research question is complected. Therefore, 
In this section, we explore data-driven methods. These methods include fine-tuning pre-trained NLP models and classical machine learning models with simple embedding. % and create an ensemble to use all of these approaches.

\subsubsection{BERT-based models}

\begin{itemize}
    \item  The BERT model \cite{devlin2018bert} is based on the Transformer \cite{vaswani2017attention}, a self-attention, encoder-decoder neural network architecture. When BERT was published in 2018, it achieved state-of-the-art results in $11$ different NLP tasks. Ever since, it has been widely used in various NLP problems \cite{young2018recent}. %As opposed to the traditional, unidirectional RNN-based language models, 
BERT is designed to learn bidirectional representations by jointly conditioning on both the left and right contexts. The basic version of BERT receives as an input a sequence of tokens of arbitrary length from a vocabulary of 30,000 tokens. %The first token of every sequence is always a special classification token ([CLS]). In addition, each logical segment of tokens is separated by the special token [SEP]. 
The output of BERT is a hidden state representation of every input token, plus a token corresponding to the aggregate sequence representation, used (for example) for classification tasks. 
\item BERT was pre-trained on Wikipedia and BooksCorpus \cite{zhu2015aligning}, which are very different from the scientific domain that we are interested in. To address this problem, we also used a variant of BERT, called SciBERT \cite{beltagy2019scibert}. SciBERT uses the same architecture as BERT, but it was optimized on scientific text. This model was pre-trained on a random sample of 1.14M papers from Semantic Scholar, containing papers from the computer science and the broad biomedical domain. 
\item Another pre-trained version of BERT is BioBERT, which is suitable for the biomedical domain \cite{lee2019biobert}. BioBERT was pre-trained on papers from PubMed, a database containing more than $30M$ citations from the biomedical literature, which makes it also a potential candidate for our purpose. 
\end{itemize}

All of the BERT-based models were fine-tuned on our dataset (technical details of the fine-tuning process are provided in section \ref{sec:pre_exp} and appendix \ref{Appendix}). %, in order to make their predictions more relevant for our task. 

\subsubsection{Classic machine learning}

We chose to include several widely used, classical machine learning models. We chose
Support Vector Machine (SVM), K-nearest neighbors (KNN) and Random Forest (RF). All models were initiated with default parameters using scikit-learn package. We used bag of words embedding as input for these models. Splits for train and test sets are presented in section \ref{sec:pre_exp}, and parameters are described in appendix \ref{Appendix}.

\subsection{Humor-Literature Inspired Classifier}
\label{subsec:HLC}

In addition to the data-driven methods, we wished to explore classifiers inspired by the humor literature (HLC). %; its input is a list of $N$ titles along with their scientific field and the output is a binary decision for each title. 
%
%based on  theoretical and empirical results in humor study.
%
We have studied extensive humor literature from sociology, psychology, cognition and neuroscience, and identified five important features, all focusing on the \emph{nouns} in the title. % as nouns capture important information regarding entities in the title, which is very relevant for our specific features. 


\textbf{Perplexity.}
\quad
Much research suggested that \emph{surprise} is a source of humor \cite{raskin1985semantic}. Indeed, we notice that titles of the Ig Nobel winners often include an unexpected term. %The unexpectedness means that these phrases are not the natural completion of the sentence. As such, they make the sentence somewhat more ambiguous. 
Consider, for example: "On the Rheology of \textbf{Cats}", "Effect of \textbf{Coke} on Sperm Motility" and "\textbf{Pigeons'} Discrimination of \textbf{Paintings} by Monet and Picasso". 

Therefore, the first type of feature we extracted measures unexpectedness. To that purpose, we used Language Models (LMs). An LM is a probability distribution over different sequences in a corpus, and thus it can be used for anomaly detection. We used LMs to measure perplexity, which is a measure from information theory, referring to how well a probability model predicts a sequence. Low perplexity indicates that the prediction of the sequence has high probability according to our LM, hence, easy to predict it (very expected).
The LM we used is N-grams, which is a probabilistic (n-1) order Markov model for predicting the next item in given a sequence. We created N-grams LMs with $n \in \{1, 2, 3\}$ for each scientific field $\in \{$neuroscience, medicine, biology, exact sciences$\}$ and uni-gram for science (all fields combined).

\textbf{Age of acquisition.} 
\quad 
Perplexity alone is insufficient; for example, the word `bremsstrahlung' (radiation emitted by the acceleration of unbound charged particles) is very unlikely to be found in an engineering corpus, but papers containing it in the title are unlikely to be funny. Rather, Ig Nobel winners tend to have relatively simple surprising words (e.g., sheep, syrup). %, or have sexual/scatological connotations. 

Thus, we defined another feature -- the noun's simplicity. According to \cite{gultchin2019humor}, simple words are more likely to be funny. Simplicity was measured using word's Age of Acquisition (AoA), a well-established measure for word's difficulty in psychology \cite{brysbaert2017test}. AoA denotes the word's difficulty according to the age a child acquires the word\footnote{Data can be found in \url{https://anonymous.4open.science/r/efd424ea-b8fc-43ae-8344-deffc418425a/}.}. 

\textbf{Word funniness level.}
\quad
%This feature is rather intuitive, as our goal is to quantify the humorous level of the title.
Some nouns are inherently funnier than others (e.g., Gobbledegook). Thus, the funniness level of nouns could correlate with the funniness of the title.   
Funniness level was measured using the model of \cite{westbury2019wriggly}, which is a linear model to quantify the funniness of single words based on rating of about 5,000 words and several humor theories. We used a data file that contained the model's rating of about $45.5K$ lemmas\footnote{Data can be found in \url{https://anonymous.4open.science/r/efd424ea-b8fc-43ae-8344-deffc418425a/}.}. %\cnote{WAY too many ``funniness/humorous level''}

\textbf{Sexual connotations.}
\quad
In line with relief theory in humor research, sexual and scatological connotations are often considered humorous \cite{shurcliff1968judged}. Examples for this feature are the past Ig Nobel winning papers ``The first case of homosexual necrophilia in the mallard anas platyrhynchos'', ``Female penis, male vagina and their correlated evolution in a cave insect'' and ``Kissing reduces allergic skin wheal responses and plasma neurotrophin levels''.

To measure sexual and scatological connotations we constructed black and white words lists. We used blacklists because while the word `sex' might be funny in the context of scientific research, it is not funny if the sentence also contains words such as `abuse', `child' or `HIV'. 


\subsubsection{Tying it all together}

%\cnote{Not sure where to put it. In the itemize itself??}

As mentioned in section \ref{sec:related_work}, Ruch proposed to divide humor into three categories: incongruity, sexual and nonsense. For our task, we can safely ignore the latter category. 
Thus, our classifier is designed to target the first two categories. 
%two prominent humor theories. 

In short, a paper is classified as funny if it has sexual and scatological connotations \cite{shurcliff1968judged}, or if it is incongruous. We define incongruity according to the general theory of verbal humor \cite{chlopicki1996linguistic}:
According to this theory, each humorous situation can be explained by two opposite scripts, which `compete' against each other to explain the situation based on cumulative evidence. Eventually, only one script can explain a given situation. This process is moderated by the use of the logical mechanism, which performs a mapping from the situation to the scripts. As long as the input (in our case, linguistic input) is well understood -- this mapping is possible. When using over-complicated terms, this mapping can go off-course, causing the miss of the humorous part in the input. For example, a paper regarding the maze navigation abilities of \emph{Ovis aries} would not be funny, but if we were to use the more common name, the title regarding \emph{sheep}'s ability to navigate in a maze would be perceived as more humorous.

We formalize this idea as follows.
A paper is classified as `funny' if it meets either of the following conditions:
\begin{itemize}
    \item The title contains a noun from the white list in the sexual connotations feature, but does not contain any of the words in the blacklist.
    \item The title contains at least one noun with a low age of acquisition and either high funniness level or high perplexity (both per field and in science combined). 
\end{itemize}{}
%For this classification, we extract five different scores for each noun in the title. If at least one of the nouns has a combination of scores which crossed the predetermined thresholds -- the whole title is classified as funny. 
To define `high' and `low', we learned the thresholds for each feature through grid search, optimizing for accuracy (see Section \ref{app:implementation_details} in appendix). %As the dataset is balanced, it is equivalent to optimizing both type one and type two errors. 
We created four different classifiers (corresponding to different sets of thresholds), one for each scientific field. %We will now present briefly the motivation and operational definition \cnote{Do CS people know this term?} behind each feature. 

Our goal in adding the literature-inspired classifier was to {\bf contrast} the common wisdom in the field of humor research with what data-driven methods could achieve. We also note that the literature-inspired classifier is easy to interpret, as opposed to the black-box machine learning models.

\subsection{Simple models} 
In addition, we considered two more simple models:

\begin{itemize}
    \item To check the hypothesis that the humor level of the words in a title is enough to indicate the title's funniness level, we used the linear regression model described in \ref{subsec:HLC} as a standalone classifier. This model was used for all nouns in a title, returning their `funniness score'. We then took the maximum over the nouns in the title to determine a single humorous level score for it. 
    % Therefore, we used \cite{gultchin2019humor}, which created a linear model to quantify the humorous level of a single word. This model is based on annotation of 120k words and features from humor literature. The score of a title is the number of funny words it contained. 
    % This score uses the humor-annotations of 120k words from \cite{gultchin2019humor}. In this paper there were three rounds of annotations, were in each round a smaller subset of the funniest words was analyzed. The last round included 216 funny words. The feature is the average number of nouns in the title that appear in the set of 215 funny words (after we removed from it the word `hippocampus', which is not funny in the scientific context). \cnote{rewrite the last part}%We then counted how many funny words each title contains, and this was and ranked the titles according to this count. 
    \item We also hypothesized that short and simple scientific titles are more likely to be perceived as funny than long and complicated ones. Thus, our readability model scores titles according to their Dale-Chall readability score \cite{dale1948formula}. The formula for this score is based on $3,000$ familiar word, classified between 4th and 13th grade level.  
\end{itemize}




\subsection{Ensemble} 
\label{ensemble}

 %Even the state-of-the-art BERT models might lack the sufficient expressivity needed for humor detection. 
%We suggest that by combining together several models, we will be able to capture more fine-grained properties, thus yielding superior results.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{overlap.png}
  \caption{Normalized overlap of the top rated 2000 paper over all scientific fields according to the different models on a random sample of papers.}
  \label{fig:overlap}
\end{figure}

%Based on the literature we know that there's great variability between the different types. With this in mind, we also explored the possibility of creating an ensemble to account for this variability. The ensemble uses all or a subset of the different models described above.
There are many ways in which a title can be funny, and assuming that a single model can handle them all might be over-optimistic.
As a quick test, we used the above-mentioned models to predict the funniness level of a \emph{random sample} of $0.5M$ papers from Semantic Scholar.
Figure \ref{fig:overlap} describes the overlap between the top 2000 rated papers according to each model (except for the literature-based models, which are binary and do not admit a ranking). We observe very low overlap between the methods. A brief manual inspection confirmed that funny papers appeared almost in all the lists. Based on those results, we decided to create an {\bf ensemble} of our models. % to combine them efficiently.

% Based on the diversity of types of humor, and the knowledge that our dataset is biased to begin with, we wondered whether accuracy on our dataset would be a sufficient measure for success. Therefore, we investigates the overlap in the prediction of the different models on a \emph{random sample} of papers from Semantic Scholar.  
%It was dome by taking a random sample of scientific papers from Semantic Scholar, and predicting the humorous level of the papers using our described above models. Then, we measured the overlap between the top 2000 rated papers according to each algorithm, leaving aside the logical rules based models, which yields binary decision rather a probability, (hence, ranking the papers is impossible). 
 %, based on the low overlap (see figure \ref{fig:overlap}). 

%An ensemble is a model, such that utilizes models' regions of speciality. 
Our ensemble (which we call `Iggy') is a \emph{stacking ensemble}: its input are the scores of each estimator, along with title features (sentence length, polarity, sentiment, AoA, percentage of difficult words, Dale Chall readability score and whether the title contains punctuation), and the scientific field. Its output is a single score, indicating the funniness of the paper.
Iggy is a multi-layer perceptron classifier (implementation details are provided in appendix \ref{Appendix}). %The pipeline of the training is presented in figure \ref{fig:pipline}. 

We first trained the models on a subset of the data and then trained the ensemble using models' predictions on a new, unseen subset. As a validation we measured the accuracy of all models and the ensemble on another subset of the data, as described in section \ref{sec:pre_exp}).

Due to the small size of our dataset and the fear of overfitting, we conducted an \emph{ablation study}, to see whether subsets of the features inserted to the ensemble can yield good enough results. We measure different subsets corresponding to the different groups of classifiers that we created (BERT-based classifiers, classical machine learning classifiers, the HLC, and the simple models) as well as any combination of the groups. All those subgroups were trained in a similar manner to the above described ensemble (implementation details can be found in appendix \ref{Appendix}). 

Only one simpler variant of the ensemble was found to perform well on the validation set; a subset with only four inputs -- scientific field, BERT, SciBERT and BioBERT. This smaller ensemble, called `BERT-Iggy', was comparable to Iggy in some fields when measuring the accuracy on our dataset.

This result is perhaps not as surprising, as BERT proved to have good, robust performance across many NLP problems. Thus, the BERT-based models inherently capture some of the literature based features. For example, perplexity is being captured by BERT, as it was designed to predict masked element in a sequence. In addition, it is also likely that the difficulty level of a word can be captured in a statistical model, as simple words are more common. %Needless to say, sexual related words should appear very rarely in corpora such as Wikipedia and BooksCorpus.
%Not to mention, 
% we wanted to see whether an ensemble that is composed solely of BERT models could achieve good performance on this highly complex task.  
 Because each one of the three BERT models could have an expertise in a different field (for example, BioBERT should have strong results on the biological and medical fields), and BERT-Iggy has access to the scientific field as input, it can be used to give more weight to each model for titles in their field of expertise.
 
After creating these ensembles (`Iggys'), we made sure they are indeed relevant by plotting the Spearman correlation matrix of all the models based on their predictions on the random sample of $0.5M$ papers (see figure \ref{fig:correlation_mat}). We can see low correlation between the predictions of the different models, which supports our hypothesis of different regions of specialisation. 

% \remove{
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=1.05\linewidth]{pipline.png}
%   \caption{Pipline of the ensemble model. Its input is the bundle of models' predictions and its output is a scalar, representing the humorous level of the title.}
%   \label{fig:pipline}
% %   https://www.draw.io/#G1AK78wxX4k4TU3dpr38KnmBmKCdaws9fp
% \end{figure}
% }



\begin{figure}[h]
  \centering
  \includegraphics[width=0.97\linewidth]{corr_mat.png}
  \caption{Spearman correlation matrix of different models.}
  \label{fig:correlation_mat}
\end{figure}
% \begin{table*}[]
% \caption{Average overlap of the top rated 2000 paper over all scientific fields according to the different models on a random sample of papers. \cnote{Find a better way to present this}}
% \label{tab:overlap_ss}
%  \begin{tabular}{l|c|c|c|c|c|c}
%       {} & KNN & RF & SVM & BERT & SCI-BERT & BIO-BERT \\ \bottomrule
% KNN & 1 & 0.029 & 0 & 0.019 & 0.022 & 0.017 \\
% RF & - & 1 & 0 & 0.106 & 0.114 & 0.189 \\
% SVM & - & - & 1 & 0.001 & 0.003 & 0 \\
% BERT & - & - & - & 1 & 0.401 & 0.105 \\
% SCI-BERT & - & - & - & - & 1 & 0.069 \\
% BIO-BERT & - & - & - & - & - & 1 \\
% \textbf{Total} & \textbf{0.181} & \textbf{0.239} & \textbf{0.167} & \textbf{0.272} & \textbf{0.268} & \textbf{0.229}
% \end{tabular}
% \end{table*}



% \subsubsection{Whole Sentence Level Features.}
% Since nouns contain much, but still limited information regarding the title, we also extracted features in the whole sentence level. This includes features such as title's scientific field, percentage of difficult words, dale chall readability score, length, sentiment, polarity and if the title contains punctuation. 


% \subsection{Architecture}

% %The model uses both features extracted based on previous literature in the field of humor, along with state-of-the-art methods in NLP (BERT, SCI-BERT). 
% Our features, since based on previous literature, contribute much for the classification task. Having that said, they are limited in the sense that they represent \emph{local} information of the title, whereas BERT represent it's \emph{holistic} information. Therefore, combining the two led to better results that also mimics human thinking better. We will shortly go into details regarding the features and architecture. 

% The initial classifier created included only the features that were extracted based on previous literature in the field of humor. As a step of improving our model we used the [CLS] output of BERT/SCI-BERT as another feature and created a FCNN. The last step of improvement was to fine-tune BERT/SCI-BERT on out dataset, to create a more appropriate [CLS] output as input for our FCNN. \cnote{not accurate... rewrite}


% \dnote{justify. why BERT?}

% % Compare to BERT's performance w.o our attention (and w.o our filtering)?? this can be our baseline

% % What about this for BERT's output? \url{https://github.com/automl/auto-sklearn}
% %\nnote{need a nice connection. I want to... mmm OK something like this:}

% %\begin{itemize}
% %    \item in the features section we will mentioned that it is possible to create a cute estimator from the features.
% %    \item however it isn't enough -- the estimator can only look at one word at a time without actually caring about the context
% %    \item we want something better that will be able to look at the context and 'understand' the title
% %    \item BERT to the rescue! it is a powerful model and many SOTAs use it as their main module
% %    \item BERT is:
% %\end{itemize}


% The BERT model \cite{devlin2018bert} is based on the Transformer \cite{vaswani2017attention}, a self-attention encoder-decoder architecture. As opposed to the traditional, unidirectional RNN-based language models, BERT is designed to learn deep bidirectional representations by jointly conditioning on both left and right context. The basic version of BERT receives as an input a sequence of tokens of arbitrary length from a vocabulary of 30,000 tokens. The first token of every sequence is always a special classification token ([CLS]). In addition, each logical segment of tokens is separated by the special token [SEP]. The output of BERT, then, is a hidden state representation of every input token, where The one corresponding to the token [CLS] is used as the aggregate sequence representation for classification tasks.

% However, BERT was pre-trained on Wikipedia and on the BooksCorpus \cite{zhu2015aligning}, which are very different from the scientific domain that we are interested in. To address this problem, we used a variant of BERT called SCI-BERT \cite{beltagy2019SCI-BERT}. SCI-BERT uses the same architecture as BERT, but it was optimized on scientific text. This model was pre-trained on a random sample of 1.14M papers from Semantic Scholar, containing papers from the computer science and the broad biomedical domain. To make SCI-BERT even more task-specific, we fine-tuned it on a corpus of 628,000 titles \cnote{change the number}. Those titles were randomly extracted from Semantic Scholar, uniformly from all fields. We used a batch size of 32, and trained the model for 8 epochs with a learning rate of 1e-7. 

% After fine-tuning SCI-BERT/BERT, we used the model to train a classifier on our dataset of funny titles. As was suggested in the original BERT paper, we added a single FC linear layer on top of the model and used a standard softmax loss. The input to this final layer is the concatenation of two vectors. The first, is the last hidden vector from the fine-tuned SCI-BERT corresponding to the first input token ([CLS]). The second, is a vector representation of the features that we extracted from the titles which were described in the features subsection. We trained the classifier for 16 epochs, using a batch size of 32 and learning rate of 5e-5 \cnote{change parameters according to the chosen model(s)}
    
% optionally, we can filter out the results using a learner that was trained on the dataset and only the features. \nnote{What do I want to say about that? I think that we need to mention the estimator in the previous section Anyway, we need to make sure that we actually use filtration}


==> modules/experiments.tex <==
After developing candidate models, we needed to evaluate them. As our labeled dataset is rather small and biased, we decided to use it only in order to filter out candidates. In section \ref{sec:ens}, we take the top candidates and evaluate them in a real-world setting. % towards the experiments. 
%These preliminary experiments were conducted on our biased, small, labeled dataset as follows. 


\subsection{Accuracy}
\label{accuracy_subsection}

We start by evaluating the models on our balanced dataset. We randomly split the data to train, ensemble-train and test sets (a $70\%-20\%-10\%$ split, respectively). We then trained the models on the train set, trained the Iggy ensembles on the train-ensemble set, and measured the accuracy on the test set. Figure \ref{fig:acc_dataset} summarizes the results. We can see that SciBERT and the two Iggys achieve the best results across the different fields. 
Noteworthy, these results are high, in an absolute sense (accuracy of $0.87-0.92$ on average). 
%However, as we noted, our dataset is small and biased, and thus we do not trust yet that these results will generalize to larger datasets.  

\begin{figure*}
  \centering
  \includegraphics[width=0.83\linewidth]{Acc_Ours_Small_Title.png}
  \caption{Accuracy of the different models on our dataset. All trainable models were trained on $70\%$ of the data. The ensembles, Iggy and BERT-Iggy, were trained on the output predictions of the trained model using $20\%$ of the data. Evaluation was done on the rest $10\%$.}
  \label{fig:acc_dataset}
\end{figure*}

\subsection{Past Ig Nobel Winners Retrieval}

On par with our initial inspiration for this study, the goal of the second experiment is to see whether the models can identify potential Ig Nobel winners. Thus, we tested whether they can retrieve past Ig Nobel Novel winners from our dataset. In this experiment, the test set was created by removing the 211 Ig Nobel winning papers from the dataset and adding a random sample of 211 negative titles, to balance the set. The remaining titles were used as a training set. This yields a non-random division of $88\%$ train and $12\%$ test set. We then further split the train set (randomly) to create a final division of $70\%-18\%-12\%$ into train, ensemble-train and test sets respectively. 

We trained the models on the train set and the ensembles on the ensemble-train set, and evaluated them by measuring their accuracy on the (new) test set. Results can be seen in figure \ref{fig:acc_ig_ret}. Similar to the finding of Section \ref{accuracy_subsection}, that SciBERT and the two Iggys achieve better results than the other models ($0.86-0.87$ on average).  

\begin{figure*}
  \centering
  \includegraphics[width=0.83\linewidth]{Igg_Acc_Small_Title.png}
  \caption{Percentage of Success Ig Nobel Retrieval. Trainable models were trained on $70\%$ of the data, the ensembles were trained on $18\%$ and accuracy was measured on $12\%$.}
  \label{fig:acc_ig_ret}
\end{figure*}

\subsection{Preliminary Conclusions}

After analyzing results of the two preliminary experiments, three models achieved superior performance across all fields -- the two ensembles and SciBERT. Therefore, we decided to use these three models for the real-world evaluation. BERT was the next best performing classifier, so we decided to test it as well (as our biased dataset might not represent the real distribution well). 

Interestingly, it appears as the literature based classifiers were indeed able to capture humor to some degree (significantly above guess level), although they did not do as well as classifiers based on BERT. %This means that humor literature was a useful implementation direction. 
As discussed in Section \ref{ensemble}, we suspect that the reason BERT was still able to achieve superior results is that it inherently captures at least some of the literature based features (for example, perplexity and level of difficulty level).  



